RAVU: Retrieval Augmented Video Understanding with Compositional Reasoning over Graph

Comprehending long videos remains a significant challenge for Large Multi-modal Models (LMMs). Current LMMs struggle to process even minutes to hours videos due to their lack of explicit memory and retrieval mechanisms. To address this limitation, we propose RAVU (Retrieval Augmented Video Understanding), a novel framework for video understanding enhanced by retrieval with compositional reasoning over a spatio-temporal graph. We construct a graph representation of the video, capturing both spatial and temporal relationships between entities. This graph serves as a long-term memory, allowing us to track objects and their actions across time. To answer complex queries, we decompose the queries into a sequence of reasoning steps and execute these steps on the graph, retrieving relevant key information. Our approach enables more accurate understanding of long videos, particularly for queries that require multi-hop reasoning and tracking objects across frames. Our approach demonstrate superior performances with limited retrieved frames (5-10) compared with other SOTA methods and baselines on two major video QA datasets, NExT-QA and EgoSchema.

==> ijcai25/3_method.tex <==
\section{Method}
\section{Method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/fig-graph-generation-cropped.pdf}
    \caption{Spatio-temporal graph generation pipeline. Firstly, LMM generates the frame description and entities for each frame extracted from the video, followed by we make entity IDs consistent across the frames. Then, we use LLM to construct the graph from them. The entity-wise events in the video are also generated to capture the segments of the video.}
    \label{fig:graph-gen}
\end{figure*}

In this section, we introduce our novel video understanding framework called \textbf{RAVU} (Retrieval Augmented Video Understanding) and discuss our approach to VideoQA through compositional reasoning over graphs in detail. 
\subsection{Overview}
Overview of our RAVU is shown in Fig.\ref{fig:overview}. RAVU consists of two primary components: the generation of spatio-temporal graphs (memory) and the application of compositional reasoning over these graphs to localize relevant video segments in response to specific queries (retrieval). These memory and retrieval mechanisms form the core of our proposed framework.

\subsection{Spatio-Temporal Graph Generation}
We represent a video as a spatio-temporal graph, where each frame is represented as a graph with entity nodes and their relationships as edges. Nodes representing the same entities across different frames are connected to incorporate the temporal dimension.    
Although there are approaches for generating scene graphs from images and videos ~\cite{sgg_survey,video_sgg_1,video_sgg_2}, they are limited by restricted vocabulary and poor generalization due to the relatively small size of the training data. We thus employ an LMM (Large Multi-modal Model) to generate frame-wise graphs and separately use the object tracklets to make temporal connections across frames. Prompting the LMM to directly identify entities, their attributes, and relationships in a frame often fails to produce high-quality graphs. To enhance the robustness of the spatio-temporal graph generation, we adopt a multi-step approach as shown in Fig.\ref{fig:graph-gen}. 

For a given video with $N$ frames, we first process each frame $x_i$ $(i=(0,...,N-1))$, using the LMM $G_l()$ with the instructions provided in the system prompt $s_{fd}$. This generates a tuple $(V_i^{'}, F_i^{'})=G_l(s_{fd}, x_i)$, where,
\begin{itemize} 
    \item $V_i^{'}$ is the set of entities $\{n_i^{j}\}$ ($j\in\{0,...,M_{i}\}$) identified in the frame-$i$. Here, $M_i$ denotes the cardinality of the set $V_i^{'}$.
    \item $F_i^{'}$ is the frame description generated by referring to the entities by their IDs.
\end{itemize} 
Each entity also has associated attributes including appearance, action, body-pose and bounding box coordinates in the entity attributes. The bounding box coordinates are necessary for tracking the entities across frames. 

% For each video frame $x^t$, we first feed it into the LMM $G_l$ to identify the entities and their attributes $V^t$ in the frame and generate the frame description by referring to the entities by their IDs. We include appearance, action, body-pose and bounding box coordinates in the entity attributes. The bounding box coordinates are necessary for tracking the entities across frames. 

% \textbf{add an equation of 1st step here}

Entity IDs in $\{(V_i^{'}, F_i^{'})\}_{i=0}^{N-1}$ are inconsistent across frames since we identify them based on a single frame. Thus, in the second step, we make them consistent based on the object tracklets to construct the temporal connections. The object tracklets can be obtained from an off-the-shelf object tracking algorithm such as ~\cite{sam2}. Let $t_i^k$, $k\in\{0,...,M-1\}$, be the $i^{th}$ frame bounding box coordinate in the tracklet of  entity-$k$ from a video with $M$ tracked entities. Then, we associate spatio temporal entity $n_i^j\in V_i^{'}$ with entity-$k$ if,
\begin{equation*}
    k=argmax_{k^{'}\in\{0,...,M-1\}}iou(t_i^{k^{'}}, n_i^j),
\end{equation*}
where $iou$ denotes the intersection-over-union. This gives us the entities set $V_i$ and $F_i$ with with entities with updated IDs  consistent across the frames. 

% $argmax_j\in{0,...,M-1}iou(n_i^{j^{'}}, T_i^j)$with the corresponding tracklets from $T_i$ by finding the tracklet bounding box having the maximum intersection-over-union (IOU) with the entity bounding box generated by the LMM in the previous step. 

% Entity IDs in the previous step are inconsistent across the frame since we identify them based on a single frame. Thus, in the second step, we make them consistent based on the tracklets to construct the temporal connections. We associate the detected entities in each frame with the corresponding tracklets. Specifically, for each entity in each frame, we find the tracklet bounding box with maximum intersection-over-union (IOU) with the entity bounding box generated by the LMM.

% \textbf{add an equation of 1st step here??}

Subsequently, for each frame, we prompt the LMM to convert the consistent frame descriptions and entities generated in the previous step to get the graph $G(V_i, E_i)=F_l(V_i, F_i, s_g)$. Here, $E_i$ contains the edges representing the relationships between the entities from the frame description $F_i$ and $s_g$ represents the system prompt with instructions for getting the graph for each frame. Note that the nodes representing entities and their attributes remain the same as previous step. Note that each node contains the rich attributes we obtained in the first step. Also, note that the prompt in this step just contains the entities and the frame description in textual format and does not include the video frame. % 

% Subsequently, to make the temporal connections, we associate the detected entities in each frame with the corresponding tracklets. Specifically, for each entity in each frame, we find the tracklet bounding box with maximum intersection-over-union (IOU) with the entity bounding box generated by the LMM.

We utilize the generated spatio-temporal graphs to identify video segments pertinent to answering a given question. Our reasoning approach on these spatio-temporal graphs involves the identification of spatio-temporal entity nodes that are most relevant to the question. To achieve this, we compute embedding of each node by computing the embedding of concise textual description of the node with a text embedding model $G_e()$. We obtain the textual description $p_i^j$ of the node $n_i^j$ as, 
\begin{equation*}
    p_i^j=G_l(n_i^j, \{e_i\}, s_d),
\end{equation*}
where, $\{e_i\}$ is the set of all edges in frame-$i$ that include  entity-$j$ and $s_d$ is the system prompt with instructions to compose a sentence that encapsulates the entity node's attributes and its relations to other entity nodes. We then compute embeddings of each node as $v_i^j=G_e(p_i^j)$.
% We utilize the generated spatio-temporal graphs to identify video segments pertinent to answering a given question. Our reasoning approach on these spatio-temporal graphs involves the identification of spatio-temporal entity nodes that are most relevant to the question. To achieve this, we employ a text-embedding model $G_e$ that, for each node $n_i^j$, embeds the phrase $p_i^j$ describing the entity node, its attributes and relations to other entities. We generate these descriptive phrases for each node by prompting the LMM to compose a sentence that encapsulates the entity node's attributes and its relations to other entity nodes. 

To facilitate temporal reasoning, we further augment the graph by creating entity-wise events. This process involves chunking the spatio-temporal nodes for each entity into distinct events, thereby capturing significant behavioral and action changes. Specifically, for the entity-$j$, we generate the events $z^j$ as 
$z^j=G_l(\{p_i^j\}_{i=0}^{N-1}, s_e)$, where the system prompt $s_e$ contains instructions to segment the node into events, capturing the entity's actions and behaviors across the frames.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/qbreakdown.png}
%     \caption{An example of our question breakdown process.}
%     \label{fig:qb}
% \end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/fig-breakdown-cropped.pdf}
    \caption{An example of our question breakdown process. LLM generates the question analysis and the sequence of reasoning steps from the input query with a few shot examples. Steps are executed sequentially from top to bottom.}
    \label{fig:qb}
\end{figure}

\subsection{Compositional Reasoning over Graph}
In this section, we present our methodology for localizing segments of a video pertinent to answering a given question by analyzing the video’s spatio-temporal graph. Our approach begins with a logical analysis of the question using an LLM to generate a sequence of reasoning steps from a predefined set, aimed at identifying the relevant video segments. To facilitate this process, we manually create examples of question analysis and breakdown for various types of questions, including temporal, descriptive, and causal, and use these examples in-context when analyzing new questions. The primary functions within our set of predefined actions include \emph{localize\_node()}, \emph{sample\_entity\_events()} and \emph{analyze\_entity\_events()}. We illustrate our question breakdown methodology through an example in Figure \ref{fig:qb}.

After breaking down the question into the sequence of reasoning steps, we perform them in sequence. The question often requires multi-step reasoning to identify the relevant frames. Specifically, if the question is "What did the man on the stage do before sitting?", the spatio-temporal entity node “man” with the attribute “man on stage sitting” must first be identified. The function \emph{localize\_node()} identifies this spatio-temporal node finding the best match of the phrase $p_g$=\emph{“man on stage sitting”} from the among the set of nodes $\{n_i^j\}$. To determine the best match, we compute the cosine similarity of each of the node embeddings $v_i^j$ with the embedding $v_g=G_e(p_g)$ of the grounding phrase. We then select the top-k spatio-temporal nodes whose embeddings exhibit the highest cosine similarity with the grounding phrase embeddings. Let $\eta=\{n_0, ..., n_{k-1}\}$ be the top-k filtered nodes and $P=\{p_0, ..., p_{k-1}\}$ be the corresponding node textual descriptions. Subsequently, we process the textual descriptions of the selected node to find the best matching node as $n_{\hat{k}}=G_l(P, p_g, s_r)$, where $s_r$ is the system prompt with instructions to select the phrase that best matches the grounding phrase and $n_{\hat{k}}$ is the best matched node. Let $n_{\hat{k}}$ correspond to the node of entity-$j$ in frame-$i$. To determine “when the man starts sitting”, the function \emph{analyze\_entity\_events()} examines the events $z_j$ of entity-$j$. This function obtains the time index $t_e$ answering the question $q_e=$\emph{“when did the man start sitting”} as $t_e=G_l(q_e, z_j, s_a)$, where $s_a$ is the system prompt containing instructions to analyse the given entity events to answer the given question. Finally, the function \emph{sample\_entity\_events()} is invoked to retrieve frames from events of entity-$j$ preceding the time index $t_e$.

